HIVE: HIerarchical Volume Encoding for Neural Implicit Surface Reconstruction

Neural implicit surface reconstruction has become a new trend in reconstructing a detailed 3D shape from images. In previous methods, however, the 3D scene is only encoded by the MLPs which do not have an explicit 3D structure. To better represent 3D shapes, we introduce a volume encoding to explicitly encode the spatial information. We further design hierarchical volumes to encode the scene structures in multiple scales. The high-resolution volumes capture the high-frequency geometry details since spatially varying features could be learned from different 3D points, while the low-resolution volumes enforce the spatial consistency to keep the shape smooth since adjacent locations possess the same low-resolution feature. In addition, we adopt a sparse structure to reduce the memory consumption at high-resolution volumes, and two regularization terms to enhance results smoothness. This hierarchical volume encoding could be appended to any implicit surface reconstruction method as a plug-and-play module, and can generate a smooth and clean reconstruction with more details. Superior performance is demonstrated in DTU, EPFL, and BlendedMVS datasets with significant improvement on the standard metrics.

==> includes/conclusion.tex <==
% \input{iclr2023/tab_fig/vis_ngp.tex}

% \input{iclr2023/tab_fig/vis_encoding.tex}

\section{CONCLUSION}
% \vspace{-3mm}
We propose to explicitly encode the 3D shape surface by hierarchical volumes to facilitate MLPs in neural implicit surface reconstruction methods. 
%In contrast to using MLPs only to encode the 3D shape information,
The spatially varying features can be obtained from high resolution volume to reason more details for each query 3D point, while the feature from low-resolution volumes could reason spatial consistency to keep shapes smooth.
We also design a sparse structure to reduce the memory consumption of high-resolution volumes, and two regularization terms to enhance surface smoothness.
Our hierarchical volume encoding could be appended to any implicit surface reconstruction method as a plug-and-play module to significantly boost their performance, which is demonstrated in three datasets.

==> includes/experiments.tex <==
\section{EXPERIMENTS}


\input{iclr2023/tab_fig/vis_dtu_blendedmvs_epfl}
\input{iclr2023/tab_fig/dtu_table}
\input{iclr2023/tab_fig/ab_all_vis}

\subsection{Implementation Details}
This work is implemented in Pytorch and experimented on Nvidia 2080Ti GPUs.
The Adam optimizer ($0.9, 0.999$) is used to update the network weights.
The learning rate for the MLPs is set to $5e^{-4}$ and decreased to ${1}/{20}$,
while the learning rates for the volumes with resolutions of $2, 4, 8, 16, 32, 64, 128, 256, 512, 1024$ are set to
% $1e^{-2},1e^{-2},1e^{-2},1e^{-2},1e^{-2},1e^{-3},1e^{-3},1e^{-4},1e^{-4},1e^{-4}$ 
$0.01,0.01,0.01,0.01,0.01,0.001,0.001,$ $1e^{-4},1e^{-4},1e^{-4}$ 
and decreased to ${1}/{100}$.
% For the high-medium-low ($1024\sim 64\sim 2$) resolutions of the volume, the learning rates are set to 1e-4, 1e-3 and 1e-2, respectively, and are reduced to $\frac{1}{100}$.
We adopt a three-stage training strategy by default, and the number of optimization iterations is set to the same as the original framework.
Taking ``NeuS + Ours" as an example, there are $300$K iterations in total. 
In the first stage, eight volumes of resolution from $[2^3,4]$ to $[256^3,4]$ are employed for $80$K-iteration optimization. 
In the second stage, a sparse volume with the resolution of $[512^3,4]$ is added for another $20$K-iteration optimization. 
Finally, a sparse volume of $[1024^3,4]$ is appended for the remaining $200$K-iteration optimization.
The length of the index tables for the second and the third stages are set to $256^3$.

% \subsection{Datasets}
% DTU~\citep{jensen2014dtudataset} is a well-used dataset for multi-view reconstruction, consisting of $124$ scans of various objects. 
% The images are obtained from an RGB camera and a structured light scanner mounted on an industrial robot arm.
% Each scene is captured from 49 or 64 views with a resolution of $1600\times 1200$.
% For a fair comparison, we follow previous methods and select 15 scenes from DTU for evaluation.
% BlendedMVS~\citep{yao2020blendedmvs} is another dataset for multi-view reconstruction composed of 113 scenes including architectures, sculptures, and small objects.
% % Each scene consists of $? - ?$ images of $768 \times 576$ pixels.
% EPFL~\cite{strecha2008epfl} is a small dataset composed of two outdoor scenes, Fountain and Herzjesu, which contain 11 and 9 high-resolution images, respectively, and the accurate ground truth meshes.



\subsection{Evaluation}
For a fair comparison, we follow previous methods to evaluate our method on DTU~\citep{jensen2014dtudataset}
, EPFL~\citep{strecha2008epfl} and BlendedMVS~\citep{yao2020blendedmvs} benchmark.
The Chamfer L1 distance is used for evaluating the accuracy of the recovered surfaces. 
This metric is the average of the accuracy, which measures the distance from the reconstructed surface to the ground-truth surface, and the completeness, which measures the distance in reverse.

We first evaluate our method on the DTU dataset and report the quantitative results in Table~\ref{tab:dtu}.
We follow previous work~\citep{darmon2022neuralwarp, oechsle2021unisurf} to clean the predicted mesh by visibility masks for more reasonable evaluation.
As shown in Table~\ref{tab:dtu}, the accuracy of previous methods is improved significantly by adding the hierarchical volume encoding.
%TODO check
To be specific, the error of NeuS~\citep{wang2021neus} is reduced by $25\% $, from $0.84$ to $0.63$, 
while the error of NeuralWarp~\citep{darmon2022neuralwarp} is reduced by $10\% $, from $0.68$ to $0.61$.
The reconstructed meshes are shown in Figure~\ref{fig:dtu blendedmvs vis}, from where we can see that the surfaces of our method are smooth and clean, while containing accurate geometry details.
For instance, the details of the house in the first scene in Figure~\ref{fig:dtu blendedmvs vis} are recovered, especially the shape of the windows and the bricks of the roof, which is more remarkable in the normal map in Figure~\ref{fig:vis normal}.

\input{iclr2023/tab_fig/epfl_table}

We then evaluate our method on the EPFL dataset.
For a fair comparison, we follow NeuralWarp to use both the ``full" chamfer distance and the ``center" chamfer distance to evaluate the reconstructed surfaces. 
The ``center" metric only evaluates the center of the scene cropped by a manually defined box,
which focuses more on the precision of the reconstruction,
while the ``full" metric is also influenced by the ground plane and the rarely seen points, which thus also considers the completeness of the reconstruction.
%% TODO: how to postprocess gt and pred mesh as done in neurewarp 
As shown in Table~\ref{tab:epfl}, the performance of each framework is improved significantly by adding our method.
Especially, the ``full" metric of NeuralWarp is decreased by $31\%$ to $5.72$, which is also a $21\%$ improvement compared to COLMAP~\citep{colmap_mvs}.


Finally, the evaluation is performed on the BlendedMVS dataset, which contains objects of more complex shapes.
As shown in Figure~\ref{fig:dtu blendedmvs vis}, our method can recover more detailed shapes than previous methods.
These illustrate that our hierarchical volume encoding can facilitate MLPs to encode more complex shapes and improve the neural implicit surface reconstruction.

%encode more complex spatial information in each voxel of the high-resolution volume, while the information encoded in the voxels of the low-resolution volume keeps the spatial consistency.


\subsection{Ablation Study}
We choose ``NeuS + Ours" to perform extensive ablation studies to validate the proposed method.
All the results are reported from the 15 scans of DTU dataset unless otherwise specified.


\textbf{Hierarchical volume encoding.}
To study the effectiveness of the hierarchical volume encoding, we equip the basic set of eight volumes to NeuS~\citep{wang2021neus} without any other change.
% We adopt $8$ thin embedding volumes with $4$ feature channels, and resolutions are from 2 to 256. Thus the largest volume's shape is $256 \times 256 \times 256 \times 4$. 
As shown in Table~\ref{tab:ab_sparse_smooth}, the error of the recovered surfaces is significantly reduced from $0.84$ to $0.70$.


\textbf{Regularization terms.}
We also ablate the two smoothness terms to study their effectiveness. As shown in  Table~\ref{tab:ab_sparse_smooth}, they help to further reduce the error metric down to $0.66$. Figure~\ref{fig:ab_all_vis} (b) shows a visual comparison without (middle) and with (right) the regularization terms. The reconstructed mesh is smoother and more complete with the regularization terms.
% As shown in Table~\ref{tab:xx}, after adding smooth terms to the optimized loss function, the reconstruction accuracy is also improved to a certain extent.
% As shown in Figure~\ref{tab:xx}, the result of the reconstructed apple will be more complete and rounded, and the geometric quality is significantly improved.


\input{iclr2023/tab_fig/ab_sparse_and_smooth}

\textbf{Sparse high resolution volume.}
We analyze the effect of the resolution of volumes.
As shown in Table~\ref{tab:ab_sparse_smooth}, sparse high resolution embedding volume (resolution of 1024 here) further improves the accuracy to $0.63$.
We also visualize the reconstructed surfaces without (left) and with (right) sparse high resolution embedding in Figure~\ref{fig:ab_all_vis}(a). It is clear that the high-resolution embedding generates more shape details, e.g., clearer facial shapes.

\input{iclr2023/tab_fig/ab_num_vol_and_res}

\textbf{Setup of embedding volumes.}
To further inspect the effect of different combinations of the volume encoding, we perform two experiments on the volume setups.
(1) We study the number of the volumes.
We first compare our hierarchical setup to a large volume of $256^3 \times 32$, the number of whose learnable parameters is about $8$ times larger than ours.
However, its performance is much worse than ours, as is presented in the left of Figure~\ref{fig:ab_num_vol_and_com_res}.
Then we keep the number of feature channels fixed at $32$ and increase the volume number. 
The resolution of the first volume is set to $256$, and the resolution of the remaining volumes is decreased by $1/2$ one by one.
As shown in Figure~\ref{fig:ab_num_vol_and_com_res} left, the accuracy of the reconstructed surface is gradually improved with the arising of the volume number.
(2) Next, we study the impact of the low-resolution volume.
We keep the resolution of the largest volume fixed at $256$, the number of the volumes fixed at $8$, and vary the resolution of the smallest volume from $2$ to $64$.
% The resolution of other volumes is interpolated in between.
The resolutions of intermediate volumes are sequentially enlarged, and the enlargement factor is $(256/min\_res)^{1/8}$.
From the results shown in Figure~\ref{fig:ab_num_vol_and_com_res} right, we can see the performance is decreased when the low-resolution volume begins from a larger resolution. This is intuitive because the low-resolution volume enforces spatial smoothness. 
Starting from a lower resolution helps to enforce smoothness across larger areas.
%This demonstrates the function of the low-resolution volume, which encodes spatial consistency from a larger space, and keep the reconstructed surface smooth.


% To verify that the spatial representation ability with multiple thin embedding volumes is strong than that of a single thick embedding volume.
% We using a single thick embedding volume with the shape of $256 \times 256 \times 256 \times 32$ to replace multiple volumes.
% Compare to multiple thin embedding volumes, the number of the learnable parameters is about $8$ times larger and the GPU memory consumption is larger.
% As shown in Table~\ref{tab:xxx}, the accuracy is worth than using multiple thin embedding volumes.
% Furthermore, We analyze the impact of the number of embedding volume.
% We keep the total embedding channel number of the concatenation is around $32$ and the number of embedding volume is set from $2$ to $9$. 
% For example, if the number of volumes is set to $4$, the channel of each volume is set to $8$.
% As shown in Table~\ref{tab:xx}, with the number of the embedding volume arises, the accuracy is also improved and become saturated gradually.

% The largest resolution affects the accuracy, and the minimum resolution also affects the accuracy. 
% If all volume embedding resolutions are from 64 to 256, this will reduce global spatial information and fail to obtain smoother reconstructions.
% To verify this, we design related experiments with different resolution combinations of embedding volumes. 
% Keep all the maximum resolution equal to 256, but the minimum resolution is from 2 to 64, the intermediate resolution is sequentially enlarged, and the enlargement factor is $(256/min\_res)^{1/8}$.
% As shown in Table~(\ref{tab:xxx}), when the minimum resolution is set to be greater than 32, the results become worse due to the lack of features which contain global information.




\textbf{Layer number of MLPs.}
Finally,  we experiment with the layer number of MLPs in the SDF network to inspect its effect.
When only half of the layers are used, the chamfer distance increases to 0.71.
More details are included in the appendix.
% The results are reported in Table~\ref{tab:xx}, from where we can see that the accuracy of our method is only rarely decreased when the number of MLPs is reduced by half.
% which also shows that our hierarchical volume encoding has more powerful representation ability.

\vspace{-3mm}
\subsection{Comparison to Hash Encoding}
% \vspace{-3mm}
A similar hierarchical feature encoding is adopted in Instant-NGP~\citep{mueller2022instant}, but the features are stored in a hash table such that the hash collision is inevitable.
This may result in cracks of the implicit geometry.
We add this hash encoding to the NeuS framework for a comparison.
According to the quantitative results in Table~\ref{tab:dtu} and the visual comparison shown in Figure~\ref{fig:ab_all_vis}(c), the quality of the reconstructed mesh with hash encoding is worse than our method.
Especially, there are many cracked areas on the reconstructed surface.
% \vspace{-3mm}





==> includes/introduction.tex <==
\section{INTRODUCTION}


\input{iclr2023/tab_fig/vis_normal}

Surface reconstruction, or image-based modeling~\citep{tan2021image}, from multi-view images is a heavily studied classic task in computer vision.
Given multiple images from different views of an object as well as the corresponding camera parameters, this task aims to recover the accurate 3D surface of the target object. Traditional methods~\citep{Fuhrmann2014} usually solve a depth map for each input image and then fuse~\citep{kazhdan2006poisson} those depth images to build a complete surface model. 
%build an energy function, and then obtain the 3D shape by minimizing this energy~\citep{colmap} with a per-scene optimization.
After the arising of deep networks, many methods try to exploit the neural networks to directly learn the mapping from 2D images to 3D surfaces~\citep{murez2020atlas,sun2021neuralrecon}.
These learning-based methods skip the intermediate depth map estimation and are highly efficient even on unseen objects and scenes. But they usually only recover coarse scale geometry and miss most of the high frequency surface details.

%ir learning from many generic scenes usually results in reconstructing only the low-frequency geometry rather than the high-frequency surface details.


Recently, many methods~\citep{idr, wang2021neus, yariv2021volsdf, darmon2022neuralwarp} have achieved highly accurate reconstruction results based on neural implicit surface. 
These methods represent the 3D shape with an implicit function, such as occupancy~\citep{oechsle2021unisurf} or signed distance fields (SDF)~\citep{wang2021neus}, and then leverage the neural radiance field (NeRF)~\citep{mildenhall2020nerf} to render the implicit geometry into color images.
Thus, the difference between the rendered images and the input images could optimize the neural radiance field as well as the implicit geometry. Strong results have been demonstrated. 
However, in these methods, the 3D shape is implicitly encoded in the multi-layer perceptrons (MLPs).
Although MLPs are compact and memory efficient, they do not have an explicit 3D structure, which may cause difficulties in learning and optimizing the target 3D shape as is observed in mesh and point-cloud processing~\citep{Chibane2020,Peng2020}.
%Sometimes, the supervision from the rendering loss could lead to ambiguous surfaces. \ping{it would be great if we can elaborate more about why it is ambiguous without our 3D feature volume}
Furthermore, it is also known~\citep{sun2021neuralrecon} that compact MLPs are hard to encode all the geometry details, such that the recovered surface is prone to be over-smooth.



% To address this problem, some methods propose to use a feature volume~\cite{} or hash tables~\cite{mueller2022instant} 

we introduce a volume encoding to facilitate an MLP to encode 3D shapes.
We represent the space with a feature volume, where the feature of each voxel encodes the 3D shape information of that location.
This structure could directly encode the geometry of each 3D position faithfully and unambiguously.
This feature encoding is then fed into an MLP to compute the SDF of an object surface.
The neural rendering process is the same as the previous method~\citep{wang2021neus},  where the rendering loss is leveraged to optimize both the MLP and our volume encoding.
To improve the  representation capability of our volume encoding, we further adopt multiple volumes of different scales.
This hierarchical structure has two advantages.
First, the high-resolution feature volume helps to reason high-frequency geometry details, while the low-resolution volume enforces spatial consistency to keep the shape smooth.
Secondly, this hierarchical structure allows us to use low-dimensional features in the high-resolution volume, which helps to reduces memory consumption. 
%a combination of multi-resolution small-width  volumes could save memory consumption compared to a high-resolution large-width volume.
%To explain why
% For example, a single large-width volume of shape $256^{3}\times32$ has approximately 8 times the amount of parameters than a multiple small-width volumes with the largest volume shape is $256^{3}\times4$.
%For example, the amount of parameters for a single large-width volume with shape of $256^{3}\times32$ has approximately 8 times of multiple small-width volumes whose amount of parameters is dominated by the largest shape volume with the shape of $256^{3}\times4$.  
To further reduce memory consumption, we sparsify high-resolution volumes with the preliminary surface reconstruction computed from low-resolution volumes. We only keep voxels nearby the surface of the preliminary results.  
Finally, we design two smoothness terms to facilitate the optimization to make the reconstructed shape clean. 
%\ping{can you add some additional description of these terms?}

In the experiments, we demonstrate that by simply adding the proposed hierarchical volume encoding, the performance of different methods are all improved significantly.
Specifically, the error of NeuS~\citep{wang2021neus} is reduced by 25\% from $0.84$ mm to $0.63$ mm, the error of VolSDF~\citep{yariv2021volsdf} is reduced by 23\% from $0.86$ mm to $0.66$ mm, and the error of NeuralWarp~\citep{darmon2022neuralwarp} is reduced by 10\% from $0.68$ mm to $0.61$ mm on the DTU~\citep{jensen2014dtudataset} dataset.
More than that, the error of NeuralWarp is reduced by 31\% on the EPFL~\citep{strecha2008epfl} dataset with the ``full" metric. 
Figure~\ref{fig:vis normal} shows an example from the DTU dataset. The color coded normal map clearly demonstrates our method can significantly boost NeuS~\citep{wang2021neus} to recover more geometry details while keeping the surface smooth and clean. 


The main contributions of this work are summarized in the following:

$\bullet$ We propose a hierarchical volume encoding, which can significantly boost the performance of neural implicit surface reconstruction as a plug-and-play module.

$\bullet$ The hierarchical volume encoding is further improved by employing a sparse structure which reduces the memory consumption, and by enforcing two regularization terms that keep the reconstructed surface smooth and clean.

$\bullet$ We demonstrate superior performance in three datasets.




==> includes/method.tex <==


\section{METHODS}


\subsection{Overview}
\input{iclr2023/tab_fig/framework}



The overall framework of our method is illustrated in Figure~\ref{fig:pipeline}.
Given multiple images $\{\mathbf{I}_{i}\}_{i=1}^{N}$ of an object and corresponding camera poses, the task is to reconstruct the 3D surface of this object.
The 3D shape is represented by an implicit SDF network, with which another implicit color network render images using the neural volume rendering.
To enhance the representation ability of the spatial information, we add a hierarchical volume encoding as the input of the SDF network, which can embed the 3D space in multiple scales.
To save the memory consumption, we also introduce a sparse structure for high-resolution volumes.
Finally, two implicit networks as well as the volume encoding are optimized by minimizing the difference between the rendered images and the input images as well as minimizing two regularization terms.


\subsection{Implicit Surface Reconstruction Based on Volume Rendering}

Neural implicit volume rendering is first introduced in \citep{mildenhall2020nerf} for novel view rendering and then used in \citep{wang2021neus, yariv2021volsdf, darmon2022neuralwarp} for surface reconstruction.
Our method could be added to any of them for better reconstruction.
Here we take NeuS~\citep{wang2021neus} as an example, which uses two multi-layer perceptrons (MLPs) to serve as two functions for representing an object: 
one is the SDF network $sdf: \mathbb{R}^3 \rightarrow \mathbb{R}$ that maps a spatial position $\mathbf{x}\in \mathbb{R}^3$ to its SDF value of the object surface, 
and the other one is the color network $c: \mathbb{R}^3 \times \mathbb{S}^2 \rightarrow \mathbb{R}$ that maps the spatial point $\mathbf{x}$ and a viewing direction $\mathbf{v}\in \mathbb{S}^2$ to a color value. 
The surface $\mathcal{S}$ is then represented by the zero-level set of the SDF function as:
\begin{equation}
    \mathcal{S} = \{\mathbf{x}\in \mathbb{R}^3 | {sdf}(\mathbf{x})=0\}.
\end{equation}

To optimize the SDF network, images are rendered from the color network as well as a weighting function computed from the SDF network.
The volume rendering function for generating colors is calculated as
\begin{equation}
    C(\mathbf{o}, \mathbf{v}) = \int_0^{+\infty}w(t)c(\mathbf{p}(t), \mathbf{v}) dt ,
\end{equation}
where $w$ is the weighting function computed by the density from the SDF network.

To make the weighting function unbiased and occlusion-aware, it is calculated as
\begin{equation}
    w(t) = T(t)\rho(t),
    \label{equ:w}
\end{equation}
where 
\begin{equation}
    T(t) = e^{-\int_0^t\rho(u)du}  ,
\end{equation}
and 
\begin{equation}
    \rho(t) = \max (\frac{-\frac{d\Phi_s}{dt}({sdf}(\mathbf{p}(t)))}{\Phi_s({sdf}(\mathbf{p}(t)))}, 0), \ \ 
    \Phi_s(x) = (1+e^{-sx})^{-1}    .
\end{equation}


\input{iclr2023/tab_fig/hierarchical_vol}

\subsection{Hierarchical Volume Encoding}

Previous methods usually encode all the information of a 3D object in the MLPs.
This works well for novel view rendering but has problems in surface reconstruction, because the simple MLP architecture makes learning and optimization inefficient.
%s do not have an explicit 3D structure. 
To address this problem, we build a 3D feature volume as the input of the MLPs, which explicitly encodes the 3D spatial information. 
This feature volume can naturally encode the knowledge about the 3D space of the object, while being optimized as well as the MLPs from the rendering loss.

To enhance the representation ability of the encoding, we also employ a hierarchical mechanism, where different scales of the 3D feature volumes are adopted, as is shown in Figure~\ref{fig:hierarchical_volume}.
In the experiments, we find a combination of multi-scale volumes works better than a single large-width volume.
This is reasonable since in low-resolution volumes, one voxel represent a large space, such that this space can have the same code.
The same code could smooth this space and prevent crushing 3D shape, which is important in surface reconstruction.

In a basic setting, we employ eight feature volumes for the 3D space encoding, whose resolutions increase from $2 \times 2 \times 2 \times 4$ to $256 \times 256 \times 256 \times 4$.
When a point $\mathbf{x}$ is being rendered, eight features of the corresponding position from these eight volumes are trilinearly interpolated and concatenated to form  $\mathcal{F}(\mathbf{x})$, which works as the input of the MLPs.
Therefore, the SDF function becomes
\begin{equation}
    \mathcal{S} = \{\mathbf{x}\in \mathbb{R}^3 | {sdf}(\mathcal{F}(\mathbf{x}))=0\}.
\end{equation}
% and the $\rho(t)$ of Equation~\ref{equ:w} becomes
% \begin{equation}
%     \rho(t) = \max (\frac{-\frac{d\Phi_s}{dt}({sdf}(\mathcal{F}(\mathbf{p}(t))))}{\Phi_s({sdf}(\mathcal{F}(\mathbf{p}(t))))}, 0).
% \end{equation}

\subsection{Sparse High Resolution Volume}
\input{iclr2023/tab_fig/sparse_table}


It is evident that the higher the resolution of the volume is, the more details would be recovered, but a volume larger than $256 \times 256 \times 256$ would consume much more memory.
To solve this problem, a multi-stage optimization scheme is adopted with high-resolution sparse volumes.
In general, a lot of voxels in a dense volume are unoccupied and invalid.
Thus, we could save memory consumption a lot by using the shape reconstructed from the coarse volumes to cull voxels far from the surface in the high-resolution volumes.

% If we can construct high resolution volume, we will get more high-frequency geometry details.
% However, when the volume resolution exceeds 256, it consume large GPU memory even if we build a thin resolution volume with few feature channels.
% To reduce memory consumption, we adopts multi-stage strategy to construct high-resolution sparse volumes.
% In general, a lot of voxels in dense volume are unoccupied and invalid.  
% We use coarse reconstructed shape result which obtained from low resolution volumes to get occupied voxels near the surface to build a sparse volume.


To do this, we propose a multi-stage optimization framework. 
In the first stage, we use the above-mentioned basic structure, where the resolution of the largest volume is $256$.
After the first stage, we obtain a coarse surface reconstruction $\mathcal{S}_c$. 
In the second stage, we utilize $\mathcal{S}_c$ to cull unnecessary voxels to obtain the valid voxels $\mathbf{V}_h^{valid}$ in the high-resolution volume.
Specifically, we first dilate the surface $\mathcal{S}_c$ to ensure all the valid voxels nearing the surface are included, where several offsets $\mathbf{dv}$ is added to each surface voxel $\mathbf{v}$ in $\mathcal{S}_c$ to get an unduplicated voxel set:
\begin{equation}
    \mathbf{V}_h^{valid} = \text{Set}(\{ \mathbf{v} + \mathbf{dv}\ |\ \mathbf{dv} \in \mathbb{Z}^3, ||\mathbf{dv}||<=r, \mathbf{v} \in \mathcal{S}_c \}).
\end{equation}
Therefore, we only need to optimize the embeddings in $\mathbf{V}_h^{valid}$ instead of all voxels.
Here, we use a simple data structure, an embedding table $T_e$, to store these embeddings.

% Specifically, we adopt a multi-stage optimization framework. In the first optimization stage, we adopt a hierarchical volume structure, where the resolution of the largest volume does not exceed 256.
% After optimized some times, we obtain a coarse mesh model $\mathbf{M}_c$ using marching cubes(). 
% We utilize $\mathbf{M}_c$ to get approximated valid voxels $\mathbf{V}_h^{valid}$ in high-resolution dense volume to construct sparse volume.
% Specifically, we first dilated mesh $\mathbf{M}_c$ to ensure the most of the surface areas are included by adding a set of integer position offsets $\mathbf{dv}$ to each vertex $\mathbf{v}$ in $\mathbf{V}_c$ obtained from $\mathbf{M}_c$ and then remove duplicate coordinates.
% \begin{equation}
%     \mathbf{V}_h^{valid} = \text{Set}(\{ \mathbf{v} + \mathbf{dv}\ |\ \mathbf{dv} \in \mathbb{Z}^3, ||\mathbf{dv}||<=r, \mathbf{v} \in \mathbf{V}_c \})
% \end{equation}
% We only need to place learnable embeddings in $V_h^{valid}$ instead of all voxels to reduce GPU memory.
% Here we use a simple data structure of embedding table $T_e$ to store these embeddings directly.

Given a floating-point three-dimensional position $\mathbf{x}$, we obtain the surrounding eight integer coordinates through the rounding operation, take out the embedding of these integer points, and then fuse them through trilinear interpolation to serve as the encoding of $\mathbf{x}$.
In order to efficiently extract the corresponding embedding from the embedding table $T_e$, we construct another index table $T_i$ which stores the indexes of $T_e$.
The values in table $T_i$ are all initialized to $-1$, which corresponds to the last embedding in table $T_e$.
Then, we assign values to table $T_i$ through the $\mathbf{V}_h^{valid}$.
Specifically, we first define a mapping function $f$: 
\begin{equation}
   f(\mathbf{x}) = x + y * N + z * N^2,
\end{equation}
where $N$ is the resolution of the volume, and $x, y, z$ are the coordinates of the position $\mathbf{x}$.
% This function $f:\mathbb{Z}^3 \rightarrow \mathbb{Z}$ can choose any form, as long as it is a 1-to-1 mapping.
We utilize $f$ to map each voxel $\mathbf{v}_j$ in $\mathbf{V}_h^{valid}$ to the index in table $T_i$, and then $T_i$ further converts it to the index $j$ in $T_e$: 
\begin{equation}
    T_i({f}(\mathbf{x})) = j,\  j = 1...n
    \label{equ:indx}
\end{equation}
where $n$ is the number of valid voxels in $\mathbf{V}_h^{valid}$. 
The length of the embedding table $T_e$ is only $n+1$ ($n \ll N^3$), such that the memory consumption is reduced a lot due to the sparse structure of the high-resolution volumes.

% After the construction of table $T_e$ is completed, it can be used directly in the subsequent optimization stage. For a batch of query 3d points, first obtain the index in batches through Equation~(\ref{equ:indx}), and then obtain the corresponding finer embedding through the index batches. As shown in Figure~(\ref{}) , finer embedding concatenate with coarse embeddings feed to MLPs together.


\subsection{Loss Function}
We equip three previous methods~\citep{wang2021neus, yariv2021volsdf, darmon2022neuralwarp} with our hierarchical volume encoding.
To optimize the model, we use the losses in their work without changes, i.e.
a rendering loss $\mathcal{L}_{color}$ which minimizes the difference between the rendered colors and input colors, and an Eikonal loss ${L_{eik}}$~\citep{icml2020eik} which encourages unit norm of  the SDF function gradients.
Besides, for NeuralWarp~\citep{darmon2022neuralwarp}, an additional warping color loss $\mathcal{L}_{warp}$ is adopted, which warps views on each other to enforce multi-view photo-consistency.

In addition, we add two additional regularization terms $\mathcal{L}_{tv}$ and $\mathcal{L}_{normal}$ to make the reconstructed surfaces smooth and clean.
The total variation (TV)~\citep{rudin1994tv} regularization is applied to each embedding volume to make adjacent voxels have similar characteristics, in which case the geometry could be more continuous and compact. It is computed as:
\begin{equation}
    \mathcal{L}_{tv} = \sum_{m} \sum_{i,j,k} \sqrt{(V_{i+1,j,k} - V_{i,j,k})^2} + \sqrt{(V_{i,j+1,k} - V_{i,j,k})^2} + \sqrt{(V_{i,j,k+1} - V_{i,j,k})^2},
\end{equation}
where $m$ is the number of the hierarchical volumes.

Another regularization term $\mathcal{L}_{normal}$ is a smoothness constraint for normal.
For each pixel of the image, we calculate the accumulated normal gradients along the marching ray as 
\begin{equation}
    N_{grad}(\mathbf{o}, \mathbf{v}) = \int_0^{+\infty}w(t)n_{grad}(t) dt ,
\end{equation}
where $n_{grad}(t)$ is the gradient of the normal at $\mathbf{p}(t)$ and computed as 
\begin{equation}
    n_{grad}(t) = \nabla^2 sdf(\mathcal{F}(\mathbf{p}(t)).
    \label{equ:n_grad}
\end{equation}
The normal regularization $\mathcal{L}_{normal}$ is then defined as:
\begin{equation}
    \mathcal{L}_{normal} = \frac{1}{N_{pix}}\sum_{pix}||N_{grad}||_2,
\end{equation}
where $N_{pix}$ is the number of pixels in one optimization. 

Thus, the final loss $\mathcal{L}$ is defined as:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{ori} + \lambda_{tv} * \mathcal{L}_{tv} + \lambda_{normal} * \mathcal{L}_{normal},
\end{equation}
where $\mathcal{L}_{ori}$ is the original loss of each method, $\lambda_{tv}$ and $\lambda_{normal}$ are two weighting factors.

% We follow the each framework \cite{wang2021neus, yariv2021volsdf, darmon2022neuralwarp} using their own loss $\mathcal{L}_{ori}$ including color loss $\mathcal{L}_{color}$ which minimize the difference between the rendered colors and ground truth colors and Eikonal loss ${L_{eik}}$ \cite{} which encourage the norm of the gradients of the SDF network output at each position to 1.  
% Besides, \cite{darmon2022neuralwarp} adopts additional warping color loss $\mathcal{L}_{warp}$ which warps views on each other to enforce multi-view photo-consistency.

% We add two additional regular terms $\mathcal{L}_{tv}$ and $\mathcal{L}_{normal}$ to make the results more smooth and better.
% The total variation (TV) \cite{} regularization is applied to each embedding volume to make adjacent voxels have similar characteristics which cause the geometry more continuous and compact. The TV loss $\mathcal{L}_{tv}$ is defined as follows:
% \begin{equation}
%     \mathcal{L}_{tv} = \sum_{n} \sum_{i,j,k} \sqrt{(V_{i+1,j,k} - V_{i,j,k})^2} + \sqrt{(V_{i,j+1,k} - V_{i,j,k})^2} + \sqrt{(V_{i,j,k+1} - V_{i,j,k})^2}
% \end{equation}
% where $n$ is the number of hierarchical volumes.

% Another regular term $\mathcal{L}_{normal}$ is the smoothness constraint for normal.
% As shown in Equation~(\ref{equ:n_grad}), the gradients of normal  $n_{grad}$ at each position $\mathbf{p}(t)$ along the viewing direction $\mathbf{v}$ calculated by the second derivative of the SDF network output.
% \begin{equation}
%     n_{grad} = \nabla^2 sdf(\mathcal{F}(\mathbf{p}(t)) 
%     \label{equ:n_grad}
% \end{equation}
% Then we accumulate the the gradients of the normal along the ray to get the normal gradient at the position $x$. The $\mathcal{L}_{normal}$ is defined as follows:
% \begin{equation}
% \begin{aligned}
%     N_{grad}(\mathbf{o}, \mathbf{v}) &= \int_0^{+\infty}w(t)n_{grad} dt \\
%     \mathcal{L}_{normal} &= \frac{1}{M}\sum_{x}||N_{grad}||_2
% \end{aligned}
% \end{equation}
% where $M$ is number of pixels participating in each optimization. The final loss $\mathcal{L}$ is defined as follows:
% \begin{equation}
%     \mathcal{L} = \mathcal{L}_{ori} + \lambda_{tv} * \mathcal{L}_{tv} + \lambda_{normal} * \mathcal{L}_{normal}
% \end{equation}


==> includes/related_work.tex <==
\section{RELATED WORK}

\textbf{Traditional multi-view surface reconstruction}
Traditional methods typically follow a long pipeline of structure-from-motion (i.e. camera calibration)~\citep{colmap_sfm}, depth map estimation~\citep{barnes2009patchmatch}, and multi-depth fusion~\citep{kazhdan2006poisson} to reconstruct surface models from images.
Many advanced geometric methods~\citep{Jiang2013,Lhuillier2005,furukawa2009accurate,galliani2015massively,colmap_mvs} have been developed to enhance these different steps in the last two decades. 
%They extract the heuristic features from the images and build a matching cost between different views, then the depths are optimized in the minimizing of the cost~\citep{colmap}.
%Afterward, an additional fusion step is needed to fuse the depths from different views to a point cloud, and then a meshing step~\citep{kazhdan2006poisson} is applied to obtain the surface.

After the arising of the deep networks, almost all steps in the conventional pipeline have been revolutionized, including feature extraction and matching~\citep{detone2018superpoint, sarlin2020superglue,tang2022quadtree}, structure-from-motion~\citep{ummenhofer2017demon,tang2018ba}, and depth map estimation \citep{yao2018mvsnet,gu2020cascade}. 

%recent methods have employed the neural networks to enhance the depth-based multi-view reconstruction.
%The modules in the traditional approaches are all improved by the deep methods, e.g., the feature extraction of the images, the matching between different views and the building of cost volume, the refinement of the 3D volume~\citep{,chen2019point,,ding2022transmvsnet}.
%But the fusion of different depth maps remains a problem.

To skip the intermediate depth map estimation, given multiple images with known camera poses, some methods try to directly regress a volumetric prediction end-to-end like an occupancy volume~\citep{ji2017surfacenet} or a TSDF volume~\citep{murez2020atlas,sun2021neuralrecon}.
While these methods simplify the overall pipeline and can be generalized to unseen objects and scenes, they often only learn to recover coarse scale geometry and miss many surface details.

%Although these methods are time-efficient and can be directly generalized to unseen objects, their network is learned from various objects. 
%By this way, the network learns the low-frequency information among various scenes, such that it can reconstruct an unseen object, but it is hard to recover the high-frequency per-scene surface details.


\textbf{Implicit surface reconstruction}
A neural radiance field (NeRF) encodes a 3D scene~\citep{mildenhall2020nerf} implicitly in a neural network. %, such that it is continuous and can achieve high spatial resolution.
The network is optimized to match the rendered images to the input images such that it can generate high quality novel view synthesis results. 
%Therefore, NeRF performs nicely in novel view synthesis.
However, since there is no constraint imposed on the 3D geometry, the surface extracted from the implicit network usually has some defects.
To address this problem, some methods first represent the 3D shape with an implicit geometry network, like occupancy grid~\citep{niemeyer2020dvr, oechsle2021unisurf} or signed distance fields~\citep{idr, wang2021neus, yariv2021volsdf, darmon2022neuralwarp, sun2022neural3dinthewild, fu2022geoneus, yu2022monosdf}, and then transfer the output of the geometry network to a density function, with which the radiance network could render color images.
In this way, the radiance network as well as the geometry network can be optimized together by matching the rendered and input images.
DVR~\citep{niemeyer2020dvr} is the first to introduce a fully differentiable renderer for implicit neural occupancy functions.
Then, IDR~\citep{idr} adds the normal and the view direction into the surface renderer, which proves their importance in disentangling geometry and appearance.
To obtain a better reconstruction, NeuS~\citep{wang2021neus} and VolSDF~\citep{yariv2021volsdf} employ the SDF representation with a volume rendering.
They model the volume density as a function of the SDF, which provides a useful inductive bias to the geometry learned in the neural volume rendering process.
Sparse-NeuS~\citep{long2022sparseneus} further tries to perform the implicit reconstruction with only sparse views, and generalizes the network to an unseen scene.
To further improve the surface quality, some methods introduce additional information, like the sparse point clouds~\citep{fu2022geoneus} or monocular depth~\citep{yu2022monosdf}, to help the reconstruction, which could recover a more detailed shape but with the cost of acquiring the additional information.

In all the above methods, however, the 3D geometry is directly encoded in the MLPs without any explicit 3D spatial information. As observed in \citep{Chibane2020,Peng2020}, the simple MLP network architecture often leads to learning and optimization difficulties and consequently inaccurate surface reconstruction.
To address this problem, we introduce a hierarchical volume encoding to explicitly encode the 3D spatial information, thus our method can reconstruct more surface details.

%an unambiguous surface could be reconstructed with rich details.



==> includes_v2/revision.tex <==
We thank all reviewers for their valuable feedback and constructive comments. We have revised the paper as suggested by the reviewers, and summarize the major revisions as follows:

- More discussion and comparison experiments to existing works about explicit (hybrid) encodings, including Plenoxels and Instant-NGP, in Section 1, Section 4, and Appendix A.6.

- More ablation study on different frameworks as a plug-in: NeuralWarp + HIVE, in Appendix A.4.

- More quantitative metrics than Chamfer distance (the normal consistency which captures the high-frequency details), in Appendix A.5

- Evaluations on novel view synthesis in Appendix A.7. 

- More discussion about the motivation and technical novelty in Section 1.

- More description of the relationship to previous works in Section 2.

- Visualization of volume encodings in Appendix A.8.

- Some minor problems.

The other concerns have also been addressed individually in the Author Responses.


==> tab_fig/ab_dtu_neuralwarp.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[h]
\centering
\small
\begin{tabular}{c c c |c}
\toprule
Hierarchical
& Regular
& Sparse
& \multirow{2}{*}{Mean} \\
Volume & Terms & High-Res &   \\
\midrule
\xmark & \xmark & \xmark & $0.68$ \\
\cmark & \xmark & \xmark & $0.64$ \\ 
\cmark & \cmark & \xmark & $0.63$ \\
\cmark & \cmark & \cmark & $0.61$ \\ 
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Ablation study of NeuralWarp+Ours on the DTU dataset.}
\label{tab:ab_neuralwarp}
% \vspace{-5mm}
\end{table}

==> tab_fig/vis_dtu_ab_neuralwarp.tex <==
\begin{figure}[h]
\centering

\begin{subfigure}{0.24\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={12cm 5cm 12cm 0cm}, clip]{figs/highres/neuralwarp/ours_low_cap_57.png}
  \caption*{Without High-res}
\end{subfigure}
%
\begin{subfigure}{0.24\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={12cm 5cm 12cm 0cm}, clip]{figs/highres/neuralwarp/ours_high_cap_57.png}
  \caption*{With High-res}
\end{subfigure}
%
\begin{subfigure}{0.24\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={10cm 3cm 8cm 3cm}, clip]{figs/smooth_term/neuralwarp/ours_nos_cap_24.png}
  \caption*{Without Regularization}
\end{subfigure}
%
\begin{subfigure}{0.24\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={10cm 3cm 8cm 3cm}, clip]{figs/smooth_term/neuralwarp/ours_cap_24.png}
  \caption*{With Regularization}
\end{subfigure}


\vspace{-2mm}
\caption{Ablation study of Neuralwarp+Ours on the DTU dataset.}
\label{fig:vis_ab_neuralwarp}
% \vspace{-5mm}
\end{figure}



==> tab_fig/vis_plenoxel.tex <==
\begin{figure}[t]
\centering


\begin{subfigure}{0.02\columnwidth}
    \small{\rotatebox{90}{~~~NeuS+Plenoxels~Image}}
\end{subfigure}
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/plenoxel_neus/img_1_42.png}
    \caption*{PSNR: $20.59$}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/plenoxel_neus/img_5_42.png}
    \caption*{PSNR: $24.14$}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/plenoxel_neus/img_30_42.png}
    \caption*{PSNR: $25.83$}
\end{subfigure}


\begin{subfigure}{0.02\columnwidth}
    \small{\rotatebox{90}{~~~NeuS+Plenoxels~Surface}}
\end{subfigure}
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/plenoxel_neus/mesh_1_42.jpg}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/plenoxel_neus/mesh_5_42.jpg}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/plenoxel_neus/mesh_30_42.jpg}
\end{subfigure}


\begin{subfigure}{0.02\columnwidth}
    \small{\rotatebox{90}{~~~~~~NeuS+Ours~~~Image}}
\end{subfigure}
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/ours/img_1_42.jpg}
    \caption*{PSNR: $21.60$}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/ours/img_5_42.jpg}
    \caption*{PSNR: $24.20$}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/ours/img_30_42.jpg}
    \caption*{PSNR: $26.09$}
\end{subfigure}


\begin{subfigure}{0.02\columnwidth}
    \small{\rotatebox{90}{~~~~~~NeuS+Ours~~~Surface}}
\end{subfigure}
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/ours/mesh_1_42.jpg}
  \caption*{10K}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/ours/mesh_5_42.jpg}
  \caption*{50K}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={6cm 0cm 0cm 3cm}, clip]{figs/compare_vol/ours/mesh_30_42.jpg}
  \caption*{300K}
\end{subfigure}



% \vspace{-1mm}
 \caption{Visual comparison to Plenoxels on DTU scan-24. The rendered novel view and the extracted mesh are displayed with respect to the iteration number.}
\label{fig:vis_plenoxel}
\vspace{-5mm}
\end{figure}


